Learning Optimal Contracts: How to Exploit Small Action Spaces

We study principal-agent problems in which a principal commits to an outcome-dependent payment scheme -- called contract -- in order to induce an agent to take a costly, unobservable action leading to favorable outcomes. We consider a generalization of the classical (single-round) version of the problem in which the principal interacts with the agent by committing to contracts over multiple rounds. The principal has no information about the agent, and they have to learn an optimal contract by only observing the outcome realized at each round. We focus on settings in which the size of the agent's action space is small. We design an algorithm that learns an approximately-optimal contract with high probability in a number of rounds polynomial in the size of the outcome space, when the number of actions is constant. Our algorithm solves an open problem by Zhu et al.[2022]. Moreover, it can also be employed to provide a $\tilde{\mathcal{O}}(T^{4/5})$ regret bound in the related online learning setting in which the principal aims at maximizing their cumulative utility, thus considerably improving previously-known regret bounds.

==> find_contract.tex <==
\subsection{The \texttt{FIND-CONTRACT} Algorithm}\label{sec:find_contract_algo}
We show now how to employ Algorithm~\ref{alg:separate_search} to design an algorithm learning an approximately contract in $\mathcal{P}$, when the number of agent's actions $n$ is a fixed parameter. As a first observation we remark that we can not directly employ Algorithm~\ref{alg:separate_search} with contract design space equal to $\preg$ as its sample complexity could be exponential in the number of states.\footnote{For example, if $\preg=[0,1]^m$ we have that the number of hyperplanes definging $\preg$ is equal to $2m$, and thus the number of samples required by Algorithm~\ref{alg:separate_search} is exponential in $m$.} To overcome this issue we invoke \separate on a larger contract design space $\mathcal{P}' \subseteq \mathbb{R}^m_{+}$ such that $ \preg \subseteq \mathcal{P}'$, defined by a number of hyperplanes $h_{\preg'}=m+1$. In such a way we efficiently identify the boundaries of the regions $\mathcal{L}_{d} \subseteq \preg'$ and the empirical distribution over outcomes associated with that regions. Subsequently, we instantiate a LP for each action $d \in \mathcal{D}$, over the set defined by the intersection of $\mathcal{L}_{d}$ and the boundaries of $\mathcal{P}$. Finally, the algorithms prescribes the principal to commit to the contract achieving the highest expected utility among the solutions returned from the LPs instantiated for each possible action $d \in \mathcal{D}$.


A crucial step in our analysis is to prove the approximate optimality of the solution returned by Algorithm~\ref{alg:final}. To do that, we tackle the challenging task of showing that if there exists an action $a \in \mathcal{A}$ that remains undiscovered during the interaction, \emph{i.e}., there is no $d \in \mathcal{D}$ such that $a \in I(d)$, then for any contract $p^* \in \mathcal{L}_{d^*} \cap \mathcal{P}_a$ for some $d^* \in \mathcal{D}$, the principal's utility is sufficiently close to the solution obtained by Algorithm~\ref{alg:final}. This is because there always a contract $p' \in \mathcal{P}_{a}$ with $a \in I(d)$ for some $d \in \mathcal{D}$ that provides a principal's utility close to the one achieved in $ p^* \in \mathcal{L}_{d^*} \cap \mathcal{P}_a$. We formalize this observation in the following lemma.

\begin{restatable}{lemma}{epsilonsolution}\label{lem:espoptsol}
The solution returned by Algorithm~\ref{alg:final} is $\mathcal{O}(\sqrt \epsilon)$-optimal.
\end{restatable}

To prove Lemma~\ref{lem:espoptsol}, we first observe that if the optimal contract is such that $p^* \in \mathcal{L}_{d} \cap \mathcal{P}_a$ for some $a \in I(d)$ with $d \in \mathcal{D}$, then the principal's estimated expected utility in $p^*$ is close to the actual one, by means of Lemma~\ref{lem:boundedactions}. On the contrary if $p^* \in \mathcal{L}_{d} \cap \mathcal{P}_a$ for an action $a \not \in I(d)$, we show that the contract $p^L = (1 -\sqrt{\epsilon}) p^* + \sqrt{\epsilon} r $ either belongs to a $\preg_{a}$ with $a \in I(d)$ for some discovered action $d \in \mathcal{D}$ or the utility estimated by the seller in $p^*$ by means of $\widetilde{F}_{d} \in \Delta_{\Omega}$ is close to the actual one. Finally, using Lemma~\ref{lem:espoptsol} and the previous lemmas, we can conclude that the solution returned by Algorithm~\ref{alg:final} is approximately optimal.

\begin{theorem}
Given $\epsilon, \alpha > 0 $, with $\mathcal{O}(\frac{n^3m^{n+1}}{\epsilon^2}\log(\frac{m}{\alpha})) $ samples the solution returned by Algorithm~\ref{alg:final} is $\sqrt{ \epsilon}$-optimal with probability of at least $1-\alpha$.
\end{theorem}

\begin{algorithm}
\caption{\texttt{FIND-CONTRACT}}
\label{alg:find_contract}
\begin{algorithmic}[1]
\Require $\alpha, \epsilon, \eta>0$ and $\mathcal{P}' \subseteq \mathbb{R}^m_{+}$
\State $\{ \mathcal{L}_{d} , \widetilde{F}_d,\}_{d \in \mathcal{D}}\leftarrow\separate (\mathcal{P}')$
\While{ $d \in \mathcal{D}$}
\State Solve the following LP:
\begin{subequations}
\begin{align*}
p_{d}^* \in \arg \max & \,\ \sum_{\omega  \in \Omega }  \widetilde{F}_{d,\omega}    \left( r_\omega - p_\omega \right)  \label{eq:utility}\\
& \text{s.t.} \quad p \in \mathcal{P} \cap \mathcal{L}_{d} 
\end{align*}
\end{subequations}
\EndWhile
\State Set $p^* \leftarrow \max_{d \in \mathcal{D}} p^*_{d}$
\State \textbf{reurn} $p^L = (1 -\sqrt{\epsilon}) p^* + \sqrt{\epsilon} r $
\end{algorithmic}
\end{algorithm}



\clearpage
\hrulefill

\subsubsection*{Event}

$\mathcal{E}_\epsilon$ is the event in which all the calls to \texttt{ACTION-ORACLE} return an $\tilde F$ such that $ \|\widetilde{F} - F_{a^\star(p)} \|_{\infty} \le \epsilon $, where $p \in \mathcal{P}$ is the contract given as input to the procedure.
%
Intuitively, \texttt{ACTION-ORACLE} works properly.

\subsubsection*{\texttt{TRY-PARTITION}}

Let $\mathcal{P}_d \subseteq \mathcal{P}$ be the set of contracts $p \in \mathcal{P}$ given as input to \texttt{ACTION-ORACLE} all the times it returned an $\tilde F$ such that $\tilde F \in \mathcal{F}_d$ (at the end of the algorithm).


Let $I(d) \coloneqq \bigcup_{p \in \mathcal{P}_d} a^\star(p)$.

\begin{lemma}
	Under $\mathcal{E}_\epsilon$, if $\tilde F = \bot$, for every discovered action $d \in \mathcal{D}$, contract $p \in \mathcal{L}_{d}$, and action $a_i \in I(d)$, it holds:
	\begin{equation*}
	\sum_{\omega \in \Omega } p_{\omega}F_{a, \omega} - c_{a} \ge
	\sum_{\omega \in \Omega } p_{\omega}F_{a', \omega} - c_{a'} -  \epsilon',
	\end{equation*}
	for every action $a' \in \mathcal{A}$, where $\epsilon' = 14 \epsilon m n$.
\end{lemma}

\begin{lemma}
	Under $\mathcal{E}_\epsilon$, if $\tilde F = \bot$, it holds:
	\[
		\bigcup_{d \in \mathcal{D}} \mathcal{L}_d = \widetilde{\mathcal{P}}.
	\]
\end{lemma}


\begin{lemma}
	Under $\mathcal{E}_\epsilon$, if $\tilde F \neq \bot$, it holds that $\left\{ d \in \mathcal{D} \mid \exists F \in \mathcal{F}_d :  \|{F} - \widetilde{F} \|_{\infty} \le 2\epsilon \right\} \neq 1$.
\end{lemma}


\subsubsection*{\texttt{UPDATE-ACTIONS}}

\begin{lemma}
	 Algorithm~\ref{alg:action_oracle} ensures that for each discovered action $d \in \mathcal{D}$ and for each actions $a_i, a_j \in I(d)$ we have $\| F_{a_i} -   F_{a_j} \|_{\infty} \le 5 \epsilon n$. Furthermore for each empirical distribution $\widetilde{F} \in \mathcal{F}_{d}$ we have: $\|\widetilde{F}- F_{a_i} \|_{\infty} \le 5 \epsilon n $ for each  $a_i \in I(d)$.
\end{lemma}

\begin{lemma}
	$I(d) \cap I(d') = \varnothing$ for every $d,d' \in \mathcal{D}$.
\end{lemma}

\subsubsection*{\texttt{FIND-CONTRACT}}

\begin{lemma}
	
\end{lemma}

\hrulefill














==> hardness.tex <==
\section{Hardness Result}
In this section we complement the study by ...  on the sample complexity of computing an approximately optimal contract. Specifically, they show that there exists an instance with $m$ outcomes and $ n = \mathcal{O} (( 1 / \epsilon) ^m) $ actions and they prove that the minimum number of samples required to learn an approximately optimal contract is of at least $\Omega ( ( 1/ \epsilon ) ^{m+2} )$. In the following we complement their study by showing that, even if the number of actions is a fixed parameter, e.g., $n=2$, the sample complexity of the computing an approximately optimal contract still depends on the the number of outcomes $m$. Specifically we show that, learning an (approximately) optimal contract requires at least $\Omega(m)$ samples as formally stated in the following.
\begin{restatable}{theorem}{hardness}
For any algorithm and for each $\epsilon > 0$, learning an $\epsilon$-optimal contracts requires at least $\Omega (m)$ samples, even with $n=2$ actions.
\end{restatable}
Theorm rules out the possibility of design an algorithm whose sample comlexity is independent from the nmber of outcomes. 

==> image.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,343); %set diagram left start at 0, and has height of 343
	
	%Straight Lines [id:da8600876828577344] 
	\draw    (155,138) -- (270,138) ;
	\draw [shift={(272,138)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Rounded Rect [id:dp23187437505266884] 
	\draw   (8,124.8) .. controls (8,120.49) and (11.49,117) .. (15.8,117) -- (79.2,117) .. controls (83.51,117) and (87,120.49) .. (87,124.8) -- (87,148.2) .. controls (87,152.51) and (83.51,156) .. (79.2,156) -- (15.8,156) .. controls (11.49,156) and (8,152.51) .. (8,148.2) -- cycle ;
	%Rounded Rect [id:dp5473179416794033] 
	\draw   (93,103.8) .. controls (93,100.6) and (95.6,98) .. (98.8,98) -- (116.2,98) .. controls (119.4,98) and (122,100.6) .. (122,103.8) -- (122,127.2) .. controls (122,130.4) and (119.4,133) .. (116.2,133) -- (98.8,133) .. controls (95.6,133) and (93,130.4) .. (93,127.2) -- cycle ;
	%Rounded Rect [id:dp3370103215028578] 
	\draw   (88,163.6) .. controls (88,160.51) and (90.51,158) .. (93.6,158) -- (110.4,158) .. controls (113.49,158) and (116,160.51) .. (116,163.6) -- (116,187.4) .. controls (116,190.49) and (113.49,193) .. (110.4,193) -- (93.6,193) .. controls (90.51,193) and (88,190.49) .. (88,187.4) -- cycle ;
	%Rounded Rect [id:dp6949824251587207] 
	\draw   (485,42.8) .. controls (485,38.49) and (488.49,35) .. (492.8,35) -- (556.2,35) .. controls (560.51,35) and (564,38.49) .. (564,42.8) -- (564,66.2) .. controls (564,70.51) and (560.51,74) .. (556.2,74) -- (492.8,74) .. controls (488.49,74) and (485,70.51) .. (485,66.2) -- cycle ;
	%Rounded Rect [id:dp09057311016356229] 
	\draw   (597,18) .. controls (597,14.13) and (600.13,11) .. (604,11) -- (632,11) .. controls (635.87,11) and (639,14.13) .. (639,18) -- (639,39) .. controls (639,42.87) and (635.87,46) .. (632,46) -- (604,46) .. controls (600.13,46) and (597,42.87) .. (597,39) -- cycle ;
	%Rounded Rect [id:dp7451308358777731] 
	\draw   (2,100.2) .. controls (2,85.18) and (14.18,73) .. (29.2,73) -- (125.8,73) .. controls (140.82,73) and (153,85.18) .. (153,100.2) -- (153,181.8) .. controls (153,196.82) and (140.82,209) .. (125.8,209) -- (29.2,209) .. controls (14.18,209) and (2,196.82) .. (2,181.8) -- cycle ;
	%Rounded Rect [id:dp5672681051149525] 
	\draw   (499.3,206.8) .. controls (499.3,202.49) and (502.79,199) .. (507.1,199) -- (570.5,199) .. controls (574.81,199) and (578.3,202.49) .. (578.3,206.8) -- (578.3,230.2) .. controls (578.3,234.51) and (574.81,238) .. (570.5,238) -- (507.1,238) .. controls (502.79,238) and (499.3,234.51) .. (499.3,230.2) -- cycle ;
	%Rounded Rect [id:dp9042496701806764] 
	\draw   (586,200.8) .. controls (586,197.6) and (588.6,195) .. (591.8,195) -- (609.2,195) .. controls (612.4,195) and (615,197.6) .. (615,200.8) -- (615,224.2) .. controls (615,227.4) and (612.4,230) .. (609.2,230) -- (591.8,230) .. controls (588.6,230) and (586,227.4) .. (586,224.2) -- cycle ;
	%Rounded Rect [id:dp10267457264113677] 
	\draw   (601,261.6) .. controls (601,258.51) and (603.51,256) .. (606.6,256) -- (623.4,256) .. controls (626.49,256) and (629,258.51) .. (629,261.6) -- (629,285.4) .. controls (629,288.49) and (626.49,291) .. (623.4,291) -- (606.6,291) .. controls (603.51,291) and (601,288.49) .. (601,285.4) -- cycle ;
	%Rounded Rect [id:dp6143714766861039] 
	\draw   (495,197.2) .. controls (495,182.18) and (507.18,170) .. (522.2,170) -- (618.8,170) .. controls (633.82,170) and (646,182.18) .. (646,197.2) -- (646,278.8) .. controls (646,293.82) and (633.82,306) .. (618.8,306) -- (522.2,306) .. controls (507.18,306) and (495,293.82) .. (495,278.8) -- cycle ;
	%Rounded Rect [id:dp4399906070419237] 
	\draw   (477,20.64) .. controls (477,10.79) and (484.99,2.8) .. (494.84,2.8) -- (639.16,2.8) .. controls (649.01,2.8) and (657,10.79) .. (657,20.64) -- (657,74.16) .. controls (657,84.01) and (649.01,92) .. (639.16,92) -- (494.84,92) .. controls (484.99,92) and (477,84.01) .. (477,74.16) -- cycle ;
	%Straight Lines [id:da41837145420537636] 
	\draw    (367,138) -- (471.4,59.2) ;
	\draw [shift={(473,58)}, rotate = 142.96] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Rounded Rect [id:dp05102690034647328] 
	\draw   (515,254.6) .. controls (515,251.51) and (517.51,249) .. (520.6,249) -- (537.4,249) .. controls (540.49,249) and (543,251.51) .. (543,254.6) -- (543,278.4) .. controls (543,281.49) and (540.49,284) .. (537.4,284) -- (520.6,284) .. controls (517.51,284) and (515,281.49) .. (515,278.4) -- cycle ;
	%Straight Lines [id:da5519628184239773] 
	\draw    (367,138) -- (485.51,244.66) ;
	\draw [shift={(487,246)}, rotate = 221.99] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	
	% Text Node
	\draw (10,128.2) node [anchor=north west][inner sep=0.75pt]    {$\ \ \ a_{1} \ a_{2} \ a_{3}$};
	% Text Node
	\draw (90,167) node [anchor=north west][inner sep=0.75pt]    {$\ a_{4}$};
	% Text Node
	\draw (95,107.2) node [anchor=north west][inner sep=0.75pt]    {$\ a_{5}$};
	% Text Node
	\draw (26,95.2) node [anchor=north west][inner sep=0.75pt]    {$\ d_{1}$};
	% Text Node
	\draw (111.4,189.4) node [anchor=north west][inner sep=0.75pt]    {$\ d_{3}$};
	% Text Node
	\draw (119,84.2) node [anchor=north west][inner sep=0.75pt]    {$\ d_{2}$};
	% Text Node
	\draw (291,129.2) node [anchor=north west][inner sep=0.75pt]    {$update\ \mathcal{D}$};
	% Text Node
	\draw (484,43.2) node [anchor=north west][inner sep=0.75pt]    {$\ \ \ a_{1} \ a_{2} \ a_{3}$};
	% Text Node
	\draw (601,19.2) node [anchor=north west][inner sep=0.75pt]    {$a_{4\ } a_{5}$};
	% Text Node
	\draw (499,14.2) node [anchor=north west][inner sep=0.75pt]    {$\ d_{1}$};
	% Text Node
	\draw (624,46.2) node [anchor=north west][inner sep=0.75pt]    {$\ d_{2}$};
	% Text Node
	\draw (148,63.2) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.82,0.01,0.11}{\ }\mathcal{D}$};
	% Text Node
	\draw (501.3,210.2) node [anchor=north west][inner sep=0.75pt]    {$\ \ \ a_{1} \ a_{2} \ a_{3}$};
	% Text Node
	\draw (603,265) node [anchor=north west][inner sep=0.75pt]    {$\ a_{4}$};
	% Text Node
	\draw (588,204.2) node [anchor=north west][inner sep=0.75pt]    {$\ a_{5}$};
	% Text Node
	\draw (516,179.2) node [anchor=north west][inner sep=0.75pt]    {$\ d_{1}$};
	% Text Node
	\draw (578.4,257.4) node [anchor=north west][inner sep=0.75pt]    {$\ d_{3}$};
	% Text Node
	\draw (612,181.2) node [anchor=north west][inner sep=0.75pt]    {$\ d_{2}$};
	% Text Node
	\draw (453,15.2) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.82,0.01,0.11}{\ }\mathcal{D}$};
	% Text Node
	\draw (465,190.2) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.82,0.01,0.11}{\ }\mathcal{D}$};
	% Text Node
	\draw (517,258) node [anchor=north west][inner sep=0.75pt]    {$\ a_{6}$};
	% Text Node
	\draw (539.4,275.4) node [anchor=north west][inner sep=0.75pt]    {$\ d_{4}$};
	
	
\end{tikzpicture}


==> regret.tex <==
\section{Drawing a connection to No-Regret Algorithms}
